Continuous Control with Deep Reinforcement Learning for Autonomous Vessels

Maritime autonomous transportation has played a crucial role in the globalization of the world economy. Deep Reinforcement Learning (DRL) has been applied to automatic path planning to simulate vessel collision avoidance situations in open seas. End-to-end approaches that learn complex mappings directly from the input have poor generalization to reach the targets in different environments. In this work, we present a new strategy called state-action rotation to improve agent's performance in unseen situations by rotating the obtained experience (state-action-state) and preserving them in the replay buffer. We designed our model based on Deep Deterministic Policy Gradient, local view maker, and planner. Our agent uses two deep Convolutional Neural Networks to estimate the policy and action-value functions. The proposed model was exhaustively trained and tested in maritime scenarios with real maps from cities such as Montreal and Halifax. Experimental results show that the state-action rotation on top of the CVN consistently improves the rate of arrival to a destination (RATD) by up 11.96% with respect to the Vessel Navigator with Planner and Local View (VNPLV), as well as it achieves superior performance in unseen mappings by up 30.82%. Our proposed approach exhibits advantages in terms of robustness when tested in a new environment, supporting the idea that generalization can be achieved by using state-action rotation.

==> sections/LiteratureReview.tex <==
\section{Related works}

\textcolor{red}{[This section still needs some work. We could divide maybe in 3 subsections.]}

\subsection{Deep Reinforcement Learning}

Deep Reinforcement learning (DRL) has been one of the most active areas of artificial intelligence in recent years, and this great wave has started by introduction of \textbf{DQN} that has achieved substantial successes on Atari games \cite{mnih2015human}. 
The  \textbf{AlphaGo} defeated the champion of Go player \cite{silver2016mastering} using general purpose reinforcement learning and planning algorithm. DRL methods have performed remarkable in traditional video games such as Super Mario Bros \cite{andrychowicz2017hindsight}, multi player games such as Quak III Arena Capture the Flag \cite{jaderberg2019human}, and strategic games like Dota \cite{pachocki2018openai}, and Starcraft ii \cite{vinyals2019grandmaster}. 

\subsection{Deep Deterministic Policy Gradient}

Along with its powerful outcomes in strategic games, the DRL has been applied on multi-goal control problems, for example Lilicrap and et. al, \cite{lillicrap2015continuous} has conducted a research over the Deep Deterministic Policy Gradient as model-free, off-policy function approximator and it was successfully performed over complex multi-joint movements, unstable and rich contact dynamics, and gait behavior. This method has been considered as a baseline for other algorithms for further development such as A3C \cite{mnih2016asynchronous} that runs DDPG method to to train the agent using multiple parallel
learners. Gu and et al. \cite{gu2017deep} proposed NAF algorithm based on the DDPG to train the the industrial Robotic arm.    
Andrychowicz et al. proposed the Hindsight Experience Replay (HER) to improve the learning process of the agent from non-desirable outcomes. Although this approach was origionally tested with DDPG, it can be combined with other off-policy RL methods whenever the multiple goals can be achieved. 

\subsection{Autonomous vessel navigation}

Along with the rapid growth of DRL models for control and robotic problems, they have been exploited for autonomous vessel navigation and ship collision avoidance. 
Sawada and et al. \cite{sawada2020automatic} employed the proximal policy optimization algorithm proposed by Schulman and et al. \cite{schulman2017proximal} in continues action space to train a model that performs automatic collision avoidance with longer safe passing distance. 
%The test environment is limited to small area without any geophraphical land and only few numbers of obstacles exist in the system. 
The trained agent were tested in different scenarios of Imazu problem with limited number of obstacles to 4 ships without any land area in the system. 
Figueiredo and et al. \cite{abou2018deep} explored Deep Deterministic Policy Gradient (DDPG) method for automated control of ships maneuvering movements in a restricted area of Suape channel. Utilizing DDPG for path planning of under-actuated surface vessels are proposed by Xue and et al. \cite{xu2019deep}. The agent is trained on a static environment with limited number of obstacles in the system. Additionally, increasing the size of these obstacles or adding land areas will result problems in the training process.       
%  \textbf{\textit{}}  
% In this work we take advantage of DDPG algorithm to train our agent such the proposed works in the X, Y , X; however, instead of feeding the parametric state-action inputs, our model uses the raw plan images. The model mimics the behavior of helmsman ,hence it only observes the raw images of the environment unlike the X, Y, Z that used the parametric-engineered inputs for the agent. This structure enables the agent to deal with the dynamic of the environment and learn the best path without any assumption on the number of moving obstacles which can be considered as the advantage of our proposed model in . Training on the raw input images will help us to operate our agent in different environments without any assumption about the geography of the environment which is the most important feature  .   

\textcolor{red}{[How do we place this work? It is the first to do what? How it is compared to others?]}









%Reinforcement learning (RL) combined with neural networks is a fundamental research topic in machine learning areas. Deep reinforcement learning (DRL) has successes in wide range of problems, such as playing Atari games\cite{mnih2013playing}\cite{mnih2015human}, Soccer simulation offense behavior\cite{hausknecht2015deep}, Playing Go\cite{silver2016mastering}, applying pick-and-place on real robot in sparse and binary rewards environment\cite{andrychowicz2017hindsight}, voyaging ship in extensive environment\cite{etemad2020using}.
Deep Reinforcement Learning (DRL) has become one of the most active research areas in Artificial Intelligence (AI). 
It has achieved outstanding success in some of the most challenging problems. 
This remarkable surge started by obtaining human-level performance in Atari games \cite{mnih2015human} without any engineered knowledge, and continued by defeating the best human player in the game of Go \cite{silver2016mastering}. 
Since then DRL has been vastly employed for robotic control \cite{gu2017deep,johannink2019residual,tai2017virtual}, strategic games \cite{cuayahuitl2015strategic,jaderberg2019human,silver2017mastering,silver2018general,vinyals2017starcraft}, natural language processing \cite{das2017learning,he2016deep,li2016deep,sharma2017literature}, and autonomous car navigation \cite{isele2018navigating,sadigh2016planning,sallab2017deep}. 
From this perspective, DRL has a strong potential to process and make decisions in challenging and dynamic environments, such as autonomous vessel navigation and collision avoidance. 

Traditionally, ship navigation has been performed entirely by humans; however, maritime technologies and AI algorithms make the automation of vessel navigation possible. 
An automated navigation system would be able to guide its operator in discovering the near-optimum trajectory for ship collision avoidance \cite{statheros2008autonomous}. 
This concept is known as path planning, in which a system attempts to find the optimal path in reaching the target point while avoiding the obstacles.% using path planning algorithms. 
The proposed algorithms in \cite{di2015energy,duchovn2014path,mac2016heuristic} require complete environmental information in the real world; this environment is mostly unknown to the agent, so considering prior knowledge for training the agent is a restricting assumption.    

% continuous environment
%     an environment that can use maps and the continuously move for the agent
% CVN = continuous vessel navigator(agent=2*CNN+DDPG) and planner and local view make
%     continuous action
%     good for long distance
%     don't need to parametrized view, it can work with some obstacles
%     can work with other maps
% SAR = States-action rotation
%     it is good for unseen and 

% The contributions of our research is divided into two parts: the simulator and the structure of agent. 
The contributions of our paper are the following.
\textcolor{blue}{First, our environment is a 2D simulation of real world maps that takes advantage of the Floyd and Ramer Douglas Peucker algorithms to find one short trajectory between two positions that doesn't intersect with lands. } 
% For the purpose of training the model in areas with presence of geographical lands we \textcolor{red}{took advantage of these algorithms'} structures \textcolor{red}{[concerning what?]}.  
\textcolor{red}{In the proposed model, the position of source and destination points can change and they are not strictly fixed locations on the map.}
% Additionally, we used the information of real world ships extracted from AIS data to simulate the dynamic of moving obstacles in the real world scenario.\textcolor{red}{previous sentence should be change, we don't have moving obstacles}  
% The agent we developed uses Deep Deterministic Policy Gradient (DDPG) and a Rotation mechanism to learn the best trajectory between any origin and destination point.
Second, the agent we developed uses Deep Deterministic Policy Gradient (DDPG) to learn the best trajectory between any origin and destination points. \textcolor{red}{what do you think about this?}\textcolor{blue}{Our proposed approach for autonomous vessel navigation using the DDPG algorithm is called Continuous Vessel Navigation with path planner and local view maker (CVN).}
In order to improve the agent's performance in unseen situations, we also propose the State-Action Rotation (SAR) strategy for preserving the obtained experiences in the replay buffer. 
To prove the strength of our model and SAR strategy, we trained our agent in the Halifax map and we tested it in Montreal, which was not previously seen by the agent. 
The obtained results suggest that our agent has a superior performance in an unseen environment with different geographical landscapes and scenarios simulated with real AIS data. 

The rest of this paper is organized as follows.
In Section \ref{sec:background} we explain concepts and terminologies that are used in this work. 
We introduce the State-Action Rotation (SAR) in Section \ref{sec:sar}, while in Section \ref{sec:basicelem} we introduce the basic elements for using reinforcement learning in a simulated vessel environment and a model called Continuous Vessel Navigator (CVN) for autonomously navigate a simulated ship from an origin to a destination. 
Section \ref{sec:exps} discuss the results of the experiments with SAR and CVN in a simulated maritime environment. 
Finally, the conclusions of this work and some research directions are shown in Section \ref{sec:conclusion}. 

%: \textcolor{red}{when we are done with editing I will fill this part.}      
% For \textcolor{red}{What are the contributions?}


% \textcolor{red}{How the paper is organized?}
% RL and DRL
% Ship Collision
% Path Planning
% Transfer Learning
% Our work
% Summary
